Time-Aware Language Models as Temporal Knowledge Bases

Many facts come with an expiration date, from the name of the President to the basketball team Lebron James plays for. But language models (LMs) are trained on snapshots of data collected at a specific moment in time, and this can limit their utility, especially in the closed-book setting where the pretraining corpus must contain the facts the model should memorize. We introduce a diagnostic dataset aimed at probing LMs for factual knowledge that changes over time and highlight problems with LMs at either end of the spectrum -- those trained on specific slices of temporal data, as well as those trained on a wide range of temporal data. To mitigate these problems, we propose a simple technique for jointly modeling text with its timestamp. This improves memorization of seen facts from the training time period, as well as calibration on predictions about unseen facts from future time periods. We also show that models trained with temporal context can be efficiently "refreshed" as new data arrives, without the need for retraining from scratch.

==> tex/exp4-representation.tex <==
\subsection{Intrinsic Evaluation}
One possible explanation for our results is that while the model has learned a joint model of text and time, it has not necessarily learned a useful model of how times relate to each other. In particular, years follow a sequence. While the calibration experiments seem to suggest the model puts higher uncertainty on further away times, this could also be explained if the model simply has seen those years less frequently. Thus, we design a diagnostic to attempt to rule out this possibility.

\paragraph{Date Comparisons}
The date comparison dataset is a very simple diagnostic dataset consisting of synthetically constructed pairs of dates. Then, the model must put the dates in order; i.e., determine whether the first date is \textit{after} or \textit{before} the second date. As a fine-tuning dataset, such a simple type of question answering has limited utility: in our baseline run, the model was able to quickly achieve 98\% accuracy. However, that a model \textit{can} learn this task does not inform us much of what the model already knows. Thus, we primarily use this dataset as a diagnostic, in order to determine whether our interventions increase a models' representation of dates in a simple but intuitive task. \je{If the accuracy is so high, is there any discriminative power by this task? Or is it not that high across the board?}

In particular, the dataset consists of several different date formats at various degrees of specificity. In a small number of cases, this can be contradicting; for instance, whether the date should be Month/Day or Day/Month cannot be disambiguated if the Day in both pairs is also a valid month. In total, there are 24 different format strings of varying levels of specificity; for instance, some may specify the day of the week or the year and others may not.

The models are then evaluated on this dataset as a cloze-style task. In particular, given a sentence like "January 24 is \blank Feburary 3rd", the model is correct if it assigns a higher probability to ``before'' than ``after''. We use this comparison as since the model does not see any training data, it may produce spurious predictions as it has not learned that the blank should always contain one of those two words.

\subsubsection*{Results}
TODO :)
